On the k-synchronizability of systems

In this paper, we work on the notion of k-synchronizability: a system is k-synchronizable if any of its executions, up to reordering causally independent actions, can be divided into a succession of k-bounded interaction phases. We show two results (both for mailbox and peer-to-peer automata): first, the reachability problem is decidable for k-synchronizable systems; second, the membership problem (whether a given system is k-synchronizable) is decidable as well. Our proofs fix several important issues in previous attempts to prove these two results for mailbox automata.

==> comparison.tex <==
% !TEX root = express19.tex

\section{Comparison with~\cite{DBLP:conf/cav/BouajjaniEJQ18}}
\label{sec:comparison}
We just showed that whether a system is \kSable{k} for a fixed $k$
is decidable, and we also showed  that the reachability problem
for \kSable{k} systems is decidable. Our proof may seem, on the surface,
quite similar to the one presented in~\cite{DBLP:conf/cav/BouajjaniEJQ18},
and it could be believed
that we only corrected a few minor typos. This section intends to expose
some of the flaws we found in~\cite{DBLP:conf/cav/BouajjaniEJQ18}
so as to defend that, on the contrary, the changes we introduced were far from
foreseeable in the original presentation.

\subsection*{Differences in the definition of $sEx_{k}(\system)$}
{\color{red}done}
%Inconsistency with the definition of $sEx_{k}(\system)$}

In \cite{DBLP:conf/cav/BouajjaniEJQ18}, Bouajjani \textit{et al.} define the set $sEx_{k}(\system)$ for a system $\system$ as the set of \kSous{k} executions of the system in the \kSous{k} semantics. Therefore, the definition of the \kSous{k} semantics of $\system$ (called $\Rightarrow_k$) is supposed to give the set $sEx_{k}(\system)$ but returns in reality concatenations of sequences of actions $e = e_1 \cdots e_n$ satisfying causal delivery such that each $e_i$ is runnable in the system. In other words, this semantics defines the set of sequences of actions with a \kSous{k} MSC, the entire sequence of actions  not necessarily being an execution of the system. For instance, the execution $e_1$ of the Example~\ref{exmp:ksynchronous}.\ref{exmp:ksable} will be recognised by the \kSous{k} semantics $\Rightarrow_k$ but this sequence of action is not runnable by the system $\system$. \todo{on peut faire plus en définissant un systeme complet }
In order to preserve the definition of a \kE{k}, we decided to consider  \kSous{k} MSC instead of \kSous{k} executions, and we defined $sEx_{k}(\system) = \{msc(e)\mid e\in\asEx_k(\system)\mbox{ and } msc(e)$  is \kSous{k}\}.
%\todo{feuille violette : erreur dans def de sExk / dans le kechange} 

\subsection*{Differences in the definition of causal delivery}
{\color{red}done}

In \cite{DBLP:conf/cav/BouajjaniEJQ18}, Bouajjani \textit{et al.}
define causal delivery verifying that messages two by two do not violate the mailbox FIFO communication. As we will see, this verification is not enough. 

\begin{example}\label{ex:counter-causal}
Let $e_1$ a sequence of actions such that $msc(e_1)$ is depicted in Figure~\ref{fig:counter-exmp-causal}a. The definition in \cite{DBLP:conf/cav/BouajjaniEJQ18} stipulates that  we should check messages with 
%\hspace*{-0.63cm}
%\begin{minipage}[b]{7.5cm}
identical receivers
 whose sends are causally related. Two pairs have to be checked: 
\begin{itemize}
\item $\send{p}{q}{\amessage_1} < \send{p}{r}{\amessage_2} < \rec{p}{r}{\amessage_2} < \send{r}{q}{\amessage_3} \in po \cup src$ and $\rec{r}{q}{\amessage_3} < \rec{p}{q}{\amessage_1} \notin po$ 
\item $ \send{r}{s}{\amessage_4} < \send{r}{t}{\amessage_5} < \rec{r}{t}{\amessage_5} < \send{t}{s}{\amessage} \in po \cup src$ and $\rec{t}{s}{\amessage_6} < \rec{r}{s}{\amessage_4} \notin po$
\end{itemize}   
 According to the definition  in \cite{DBLP:conf/cav/BouajjaniEJQ18}, this MSC satisfies causal delivery. However, it seems to be obvious that it does not exist an execution corresponding to this; indeed it is impossible to linearise this partial order. Due to this, we check that a total order is possible from the partial order in our definition of causal delivery. 

In the other hand, we can easily see that the original definition aims to verify that the mailbox is well respected. However,  some causally dependencies are missing.

 Let $e_2$ a sequence of actions such that $msc(e_2)$ is depicts in Figure~\ref{fig:counter-exmp-causal}b. As previously, we are supposed to check only messages with identical receiver and whose sends are causally dependent: 
%\end{minipage}
%\begin{minipage}[b]{6cm}
%\end{minipage}
%\todo{cahier : erreur dans def causal deliver x2}
\begin{itemize}
\item $\send{p}{q}{\amessage_3} < \send{p}{r}{\amessage_4} < \rec{p}{r}{\amessage_4} < \send{r}{q}{\amessage_5} \in po \cup src$ and $\rec{r}{q}{\amessage_5} < \rec{p}{q}{\amessage_3} \notin po$
\end{itemize}
According to the original definition, this MSC respects causal delivery. However, it ignores the dependence between $\amessage_2$ and $\amessage_3$. Indeed, the mailbox communication implies that if $\rec{t}{q}{\amessage_2} < \rec{p}{q}{\amessage_3}$ with the same receiver then $\send{t}{q}{\amessage_2} < \send{p}{q}{\amessage_3}$. With this new constraint, it is impossible to find a linearisation from this partial order. We can deduce that their definition of causal relation is not complete enough and should also consider the order imposed by the mailbox communication; in this case, a causally dependence would have been detected between $\amessage_1$ and $\amessage_6$ and we would have seen that the receptions did not correspond to the receives. 
\end{example}
\begin{figure}
\begin{center}
\begin{tikzpicture}[scale = 0.7]
\begin{scope}
\draw (2,-4.8) node[above] {$\textbf{(a)}$};
\draw (0,0.2) node[above]{$p$} ;
\draw (1,0.2) node[above]{$q$}; 
\draw (2,0.2) node[above]{$r$};
\draw (3,0.2) node[above]{$s$};
\draw (4,0.2) node[above]{$t$};
\draw (0,0.2) edge (0,-3.8); 
\draw (1,0.2) edge (1,-3.8);
\draw (2,0.2) edge (2,-3.8); 
\draw (3,0.2) edge (3,-3.8); 
\draw (4,0.2) edge (4,-3.8);
\draw[>=latex, ->] (0,-0.5) to node [pos = 0.7, above, scale = 0.9] {$\amessage_1$} (1,-0.5);
\draw[>=latex, ->] (0,-1) to node [above, sloped, pos = 0.2, scale = 0.9] {$\amessage_2$} (2,-1);
\draw[>=latex, ->] (2,-1.5) to node [above, scale = 0.9, pos=0.3] {$\amessage_3$} (1,-1.5);
\draw[>=latex, ->] (2,-2) to node [above, scale = 0.9] {$\amessage_4$} (3,-2);
\draw[>=latex, ->] (2,-2.5) to node [above, scale = 0.9,pos=0.7] {$\amessage_5$} (4,-2.5);
\draw[>=latex, ->] (4,-3) to node [above, scale = 0.9] {$\amessage_6$} (3,-3);
\draw[>=latex, ->] (4,-3.5) to node [below, pos = 0.1, scale = 0.9] {$\amessage_7$} (0,0);
\end{scope} 

\begin{scope}[xshift = 6.5cm]
\draw (2,-4.8) node[above] {$\textbf{(b)}$};
\draw (0,0.2) node[above]{$p$} ;
\draw (1,0.2) node[above]{$q$}; 
\draw (2,0.2) node[above]{$r$};
\draw (3,0.2) node[above]{$s$};
\draw (4,0.2) node[above]{$t$};
\draw (0,0.2) edge (0,-3.8); 
\draw (1,0.2) edge (1,-3.8);
\draw (2,0.2) edge (2,-3.8); 
\draw (3,0.2) edge (3,-3.8); 
\draw (4,0.2) edge (4,-3.8);
\draw[>=latex, ->] (4,-0.5) to node [pos = 0, right, scale = 0.9] {$\amessage_1$} (3,-3.5);
\draw[>=latex, ->] (4,-1) to node [above, sloped, pos = 0.5, scale = 0.9] {$\amessage_2$} (1,-1);
\draw[>=latex, ->] (0,-1.5) to node [above, scale = 0.9, pos=0.5] {$\amessage_3$} (1,-1.5);
\draw[>=latex, ->] (0,-2) to node [above, scale = 0.9, pos=0.25] {$\amessage_4$} (2,-2);
\draw[>=latex, ->] (2,-2.5) to node [above, scale = 0.9,pos=0.5] {$\amessage_5$} (1,-2.5);
\draw[>=latex, ->] (2,-3) to node [above, scale = 0.9] {$\amessage_6$} (3,-3);
%\draw[>=latex, ->] (4,-3.5) to node [below, pos = 0.1, scale = 0.9] {$\amessage_7$} (0,0);
\end{scope} 

\end{tikzpicture}
\end{center}
\caption{MSCs violating
causal delivery}
\label{fig:counter-exmp-causal}
\end{figure}


\subsection*{Differences in the graphical characterisation of \kSable{k}
  executions}
  {\color{red}done} 

In \cite{DBLP:conf/cav/BouajjaniEJQ18}, Bouajjani \textit{et al.}
%define  synchronizability for mailbox systems.
give the following characterisation of \kSous{k} executions in terms of a
structural property of the conflict graphs of their MSC.

\begin{quote}
{\bf Characterisation of \kSity{k}~\cite[Theorem~1]{DBLP:conf/cav/BouajjaniEJQ18}.} A MSC $t$\footnote{A trace $t$, as in the original terminology.} satisfying causal delivery is \kSous{k} iff every \emph{cycle} in its conflict graph does not contain a $RS$ edge and is of size at most $k$.
\end{quote}

If the word \emph{cycle} in this statement means
\emph{Hamiltonian cycle} (i.e., a cyclic path that does not go twice
through the same vertex), then this statement is not correct. Indeed,
consider again Example~\ref{ex:counter-exmp-SCC}. This graph is not Hamiltonian,
and the largest Hamiltonian cycle indeed is of size 4 only. But as we already
discussed in Example~\ref{ex:counter-exmp-SCC}, the corresponding MSC is not
\kSous{4}. 

It is true that the word cycle could be understood, with some open mindedness,
as equivalent to SCC. But the subsequent developments
in~\cite{DBLP:conf/cav/BouajjaniEJQ18}
indicate that what is meant by \emph{cycle} in the above statement
really is Hamiltonian cycle. In particular, the algorithm that is
later used for deciding whether a system is \kSable{k} is not correct
either: the MSC of Figure~\ref{fig:ex-counter-exmp-SCC}c would
be considered as \kSable{4} according to this algorithm.  


\subsection*{Differences in the definition of $\transitionKE{e}{k}$}
{\color{red}done}

In \cite{DBLP:conf/cav/BouajjaniEJQ18} the authors define
$\transitionKE{e}{k}$ in a rather different way:
they do not explicitly
give a graphical characterisation of causal delivery; instead they compute,
for every process $p$, the set $B(p)$ of processes that either
sent an unmatched message to $p$ or received a message
from a process in $B(p)$. They then make sure that any message sent to $p$ by
a process $q\in B(p)$ is unmatched.
According to that,
 relation $\transitionKE{e}{k}$ in \cite{DBLP:conf/cav/BouajjaniEJQ18},
considers that
the following execution (see also Example~\ref{ex:causal-delivery})
\begin{align*}
&\send{q}{r}{\amessage_1}\cdot\send{q}{s}{\amessage_2}\cdot\rec{q}{s}{\amessage_2}
\cdot\send{p}{s}{\amessage_3}\cdot\rec{p}{s}{\amessage_3}\cdot \\
&\send{p}{r}{\amessage_4}\cdot\rec{p}{r}{\amessage_4}
\end{align*}
satisfies causal delivery and is \kSous{1}.
However, this is not the case:  we saw in Example~\ref{ex:causal-delivery} that
neither this execution nor any causally equivalent satisfy causal delivery.

\subsection*{Differences in the definition of $\transitionCD{e}{k}$}
{\color{red}done} 

In \cite{DBLP:conf/cav/BouajjaniEJQ18} the authors verify that a trace is feasible with a \emph{monitor} which reviews the actions of the execution and adds processes that no longer are allowed to send a message to the receiver of $\pi$, in the same way as function $B$. According to this monitor, the following execution $e' = \deviate{e \cdot r} $ (MSC in Figure~\ref{fig:problematic-exe}a) is feasible, i.e., is runnable in $\system'$ and $e \cdot r$ is runnable in $\system$. 
\begin{align*}
e' =~  & \send{q}{\pi}{(r,\amessage_1)}\cdot\rec{q}{\pi}{(r,\amessage_1)}\cdot
\send{q}{s}{\amessage_2}\cdot\rec{q}{s}{\amessage_2}
\cdot \\ 
& \send{p}{s}{\amessage_3}\cdot\rec{p}{s}{\amessage_3}\cdot \send{p}{r}{\amessage_4}\cdot\rec{p}{r}{\amessage_4} \cdot  \\
& \send{\pi}{r}{\amessage_1}\cdot\rec{\pi}{r}{\amessage_4}
\end{align*}

However, as previously, this execution is not feasible because there is a causal dependency between $\amessage_1$ and $\amessage_3$. 
This execution would then be considered as feasible and therefore would belong to set $sTr_k(\system')$. As there is no corresponding execution in $asTr(\system)$, the comparison and therefore the \kSity{k}, could be distorted and appear as a false negative. 


\subsection*{Differences in the definition of $\transitionBV{e}{k}$}
{\color{red} done} 

As for the notion of feasibility, to determine if an execution is bad,  in \cite{DBLP:conf/cav/BouajjaniEJQ18} the authors use a monitor that builds a path between the send to process $\pi$ and the send from $\pi$. 
In addition to the problems related to the wrong characterisation of \kSity{k}, this monitor not only
can detect  an $RS$ edge  when there should be none, but also it can miss them when they exist. In general, the problem arises because the path is constructed by considering only an endpoint at the time (see Example~\ref{ex:counter-bad-def} in Appendix~\ref{sec:additional} for more explanations). 

\begin{example}\label{ex:counter-bad-def}
Figure~\ref{fig:problematic-exe}b depicts the MSC associated to an execution feasible and without label $RS$. Still, the monitor considers the reception of $\amessage_2$ followed by the send of $\amessage_3$. A label $RS$ is thus wrongly detected. 
Conversely, Figure~\ref{fig:problematic-exe}c depicts the MSC associated to an execution feasible but bad. With the monitor  in \cite{DBLP:conf/cav/BouajjaniEJQ18}, the action seen after the send of $\amessage_3$ is the send of $\amessage_4$ and so the existing label $RS$ is ignored at the profit of a non existing  label $SS$.  
\end{example}


\begin{figure}

\begin{center}

\begin{tikzpicture}[scale = 0.8,every node/.style={scale=0.8}]


\begin{scope}
	%MACHINE
	\coordinate(Aa) at (0,0) ;
	\coordinate (Ab) at (0,-3) ;
	\coordinate (Ba) at (1,0) ;
	\coordinate (Bb) at (1,-3) ;
	\coordinate (Ca) at (2,0) ;
	\coordinate (Cb) at (2,-3) ;
	\coordinate (Pa) at (3,0) ;
	\coordinate (Pb) at (3,-3) ;
	\coordinate (Da) at (4,0) ;
	\coordinate (Db) at (4,-3) ;
	\draw (Aa) node[above]{$p$} ;
	\draw (Ba) node[above]{$q$} ;
	\draw (Ca) node[above]{$r$} ;
	\draw (Pa) node[above]{$s$} ;
	\draw (Da) node[above]{$\pi$} ;
	\draw (Aa) -- (Ab) ;
	\draw (Ba) -- (Bb) ;
	\draw (Ca) -- (Cb) ;
	\draw (Pa) -- (Pb) ;
	\draw (Da) -- (Db) ;
	%MESSAGES 
	\coordinate (sa) at (1,-0.5); 
	\coordinate (ra) at (4,-0.5); 
	\draw[>=latex,->] (sa) to node[above, sloped, pos = 0.17]{$(r,\amessage_1)$}(ra);
	
	\coordinate (sb) at (1, -1); 
	\coordinate (rb) at (3, -1); 
	\draw[>=latex,->] (sb) -- (rb); 
	\draw (sb) node[above right]{$\amessage_2$} ;
	
	\coordinate (sc) at (0, -1.5); 
	\coordinate (rc) at (3, -1.5); 
	\draw[>=latex,->] (sc) -- (rc); 
	\draw (sc) node[above right]{$\amessage_3$};

	\coordinate (sd) at (0, -2); 
	\coordinate (rd) at (2, -2); 
	\draw[>=latex,->] (sd) -- (rd); 
	\draw (sd) node[above right]{$\amessage_4$};
	
	\coordinate (sd) at (4, -2.5); 
	\coordinate (rd) at (2, -2.5); 
	\draw[>=latex,->] (sd) -- (rd); 
	\draw (sd) node[above left]{$\amessage_1$};
	
	\draw (2,-4) node[above]{\textbf{(a)}};
\end{scope}

\begin{scope}[shift = {(6,0)}]
	%MACHINE
	\coordinate(Aa) at (0,0) ;
	\coordinate (Ab) at (0,-3) ;
	\coordinate (Ba) at (1,0) ;
	\coordinate (Bb) at (1,-3) ;
	\coordinate (Ca) at (2,0) ;
	\coordinate (Cb) at (2,-3) ;
	\coordinate (Pa) at (3,0) ;
	\coordinate (Pb) at (3,-3) ;
	\draw (Aa) node[above]{$p$} ;
	\draw (Ba) node[above]{$q$} ;
	\draw (Ca) node[above]{$r$} ;
	\draw (Pa) node[above]{$\pi$} ;
	\draw (Aa) -- (Ab) ;
	\draw (Ba) -- (Bb) ;
	\draw (Ca) -- (Cb) ;
	\draw (Pa) -- (Pb) ;
	%MESSAGES 
	\coordinate (sa) at (0,-0.5); 
	\coordinate (ra) at (3,-0.5); 
	\draw[>=latex,->] (sa) to node[above, sloped, pos = 0.17]{$(r,\amessage_1)$} (ra); 
	
	\coordinate (sb) at (0, -1); 
	\coordinate (rb) at (1, -1); 
	\draw[>=latex,->] (sb) -- (rb); 
	\draw (sb) node[above right]{$\amessage_2$};
	
	\coordinate (sc) at (2, -1.5); 
	\coordinate (rc) at (1, -1.5); 
	\draw[>=latex,->] (sc) -- (rc); 
	\draw (sc) node[above left]{$\amessage_3$};

	\coordinate (sd) at (3, -2); 
	\coordinate (rd) at (2, -2); 
	\draw[>=latex,->] (sd) -- (rd); 
	\draw (sd) node[above left]{$\amessage_1$};
	
	\draw (1.5,-4) node[above]{\textbf{(b)}};
\end{scope}



\begin{scope}[shift = {(11,0)}]
	%MACHINE
	\coordinate(Aa) at (0,0) ;
	\coordinate (Ab) at (0,-3) ;
	\coordinate (Ba) at (1,0) ;
	\coordinate (Bb) at (1,-3) ;
	\coordinate (Ca) at (2,0) ;
	\coordinate (Cb) at (2,-3) ;
	\coordinate (Pa) at (3,0) ;
	\coordinate (Pb) at (3,-3) ;
	\draw (Aa) node[above]{$p$} ;
	\draw (Ba) node[above]{$q$} ;
	\draw (Ca) node[above]{$r$} ;
	\draw (Pa) node[above]{$\pi$} ;
	\draw (Aa) -- (Ab) ;
	\draw (Ba) -- (Bb) ;
	\draw (Ca) -- (Cb) ;
	\draw (Pa) -- (Pb) ;
	%MESSAGES 
	\coordinate (sa) at (0,-0.5); 
	\coordinate (ra) at (3,-0.5); 
	\draw[>=latex,->] (sa) to node[above, sloped, pos = 0.17]{$(r,\amessage_1)$} (ra); 
	
	\coordinate (sb) at (0, -1); 
	\coordinate (rb) at (1, -1); 
	\draw[>=latex,->] (sb) -- (rb); 
	\draw (sb) node[above right]{$\amessage_2$};
	
	\coordinate (sc) at (1, -1.5); 
	\coordinate (rc) at (0, -1.5); 
	\draw[>=latex,->] (sc) to node[above,pos=0.8]{$\amessage_3$} (0.65,-1.5); 
	\draw[>=latex, ->, dashed] (0.65,-1.5)--(rc); 
	%\draw (sc) node[above right]{$\amessage_3$};
	
	\coordinate (sd) at (2, -2); 
	\coordinate (rd) at (1, -2); 
	\draw[>=latex,->] (sd) -- (rd); 
	\draw (sd) node[above left]{$\amessage_4$};

	\coordinate (se) at (3, -2.5); 
	\coordinate (re) at (2, -2.5); 
	\draw[>=latex,->] (se) -- (re); 
	\draw (se) node[above left]{$\amessage_1$};
	
		\draw (1.5,-4) node[above]{\textbf{(c)}};

\end{scope}
\end{tikzpicture}
\caption{MSCs of problematic executions}\label{fig:problematic-exe}
\end{center}

\end{figure}
\subsection*{Other differences}
\todo{a ajouter qqpart} 

Due to to the above errors, that concern fundamental points
in \cite{DBLP:conf/cav/BouajjaniEJQ18}, we had to propose a considerably different approach. %introduce a lot of new material. 
The extended edges of the conflict graph, and the
graphical characterisation of causal delivery as well as summary nodes, have no equivalent in
\cite{DBLP:conf/cav/BouajjaniEJQ18}.
As underlined above,  transition relations $\transitionCD{e}{k}$ and $\transitionBV{e}{k}$ build on the graphical characterisations of causal delivery and \kSity{k}, they depart considerably from  the proposal in \cite{DBLP:conf/cav/BouajjaniEJQ18}.



%And, as previously said, the transition relations $\transitionCD{e}{k}$ and $\transitionBV{e}{k}$ also 
%have been completely reconsidered from
%have nothing in common with the 
%corresponding relations in~\cite{DBLP:conf/cav/BouajjaniEJQ18}.
% : these relations build on the graphical characterizations of causal delivery and \kSity{k}, so they had to be entirely reconsidered from scratch.


==> exemple_long.tex <==
\begin{tikzpicture} 
\begin{scope}
%MACHINE
  \coordinate(pa) at (0,-0.5) ;
  \coordinate (pb) at (0,-5.5) ;
  \coordinate (qa) at (0.5,-0.5) ;
  \coordinate (qb) at (0.5,-5.5) ;
  \coordinate (ra) at (1,-0.5) ;
  \coordinate (rb) at (1,-5.5) ;
  \coordinate (sa) at (1.5,-0.5) ;
  \coordinate (sb) at (1.5,-5.5) ;
  \coordinate (ta) at (2,-0.5) ;
  \coordinate (tb) at (2,-5.5) ;
  \coordinate (ua) at (2.5,-0.5) ;
  \coordinate (ub) at (2.5,-5.5) ;


  \draw (pa) node[above]{$p$} ;
  \draw (qa) node[above]{$q$} ;
  \draw (ra) node[above]{$r$} ;
  \draw (sa) node[above]{$s$} ;
  \draw (ta) node[above]{$t$} ;
  \draw (ua) node[above]{$u$} ;
  \draw (pa) -- (pb) ;
  \draw (qa) -- (qb) ;
  \draw (ra) -- (rb) ;
  \draw (sa) -- (sb) ;
  \draw (ta) -- (tb) ;
  \draw (ua) -- (ub) ;
  
  %MESSAGES 
  \coordinate (s1) at (0.5, -1); 
  \coordinate (m1) at (0.9, -1);
  \coordinate (r1) at (1.5, -1); 
  \draw[>=latex,->] (s1) -- (m1) node[midway, above] {$\amessage_1$};
	\draw[>=latex,->,dashed] (m1) -- (r1);
  
  \coordinate (s2) at (0.5, -1.5); 
  \coordinate (r2) at (2, -1.5); 
  \draw[>=latex, ->] (s2) -- (r2); 
  \draw (s2) node[above right]{$\amessage_2$};
 
  \coordinate (s3) at (2, -2.5); 
  \coordinate (r3) at (0, -2.5); 
  \draw[>=latex, ->] (s3) -- (r3); 
  \draw (s3) node[above left]{$\amessage_3$};

  \coordinate (s4) at (2.5, -3); 
  \coordinate (r4) at (0, -3); 
  \draw[>=latex, ->] (s4) -- (r4); 
  \draw (s4) node[above left]{$\amessage_4$};
  
  \coordinate (s5) at (1, -4); 
  \coordinate (r5) at (2.5, -4); 
  \draw[>=latex, ->] (s5) -- (r5); 
  \draw (s5) node[above right]{$\amessage_5$};  
  
  \coordinate (s6) at (2.5, -5); 
  \coordinate (r6) at (1.5, -5); 
  \draw[>=latex, ->] (s6) -- (r6); 
  \draw (s6) node[above left]{$\amessage_6$};    
  
  %K-ECHANGES 
  	%dans msc
	\coordinate (km1a) at (-0.5,-2); 
	\coordinate (km1b) at (3,-2); 
	\draw[dashed] (km1a) -- (km1b);
	%dans graph
	\coordinate (kg1a) at (5,-2); 
	\coordinate (kg1b) at (13,-2); 
	\draw[dashed] (kg1a) -- (kg1b);
	%accolade
	\coordinate (acc1b) at (-0.5,-0.5); 
	\coordinate (acc1a) at (-0.3,-0.5); 
	\coordinate (acc1c) at (-0.5,-1.9); 
	\coordinate (acc1d) at (-0.3,-1.9); 
	\draw (acc1a) -- (acc1b) -- (acc1c)node[midway, left]{$e_1$} -- (acc1d);	
	  
	%dans msc
	\coordinate (km2a) at (-0.5,-3.5); 
	\coordinate (km2b) at (3,-3.5); 
	\draw[dashed] (km2a) -- (km2b);
	%dans graph
	\coordinate (kg2a) at (5,-3.5); 
	\coordinate (kg2b) at (13,-3.5); 
	\draw[dashed] (kg2a) -- (kg2b);
	%accolade
	\coordinate (acc2b) at (-0.5,-2.1); 
	\coordinate (acc2a) at (-0.3,-2.1); 
	\coordinate (acc2c) at (-0.5,-3.4); 
	\coordinate (acc2d) at (-0.3,-3.4); 
	\draw (acc2a) -- (acc2b) -- (acc2c)node[midway, left]{$e_2$} -- (acc2d);
	
	
	%dans msc
	\coordinate (km3a) at (-0.5,-4.5); 
	\coordinate (km3b) at (3,-4.5); 
	\draw[dashed] (km3a) -- (km3b);
	%dans graph
	\coordinate (kg3a) at (5,-4.5); 
	\coordinate (kg3b) at (13,-4.5); 
	\draw[dashed] (kg3a) -- (kg3b);
	%accolade
	\coordinate (acc3b) at (-0.5,-3.6); 
	\coordinate (acc3a) at (-0.3,-3.6); 
	\coordinate (acc3c) at (-0.5,-4.4); 
	\coordinate (acc3d) at (-0.3,-4.4); 
	\draw (acc3a) -- (acc3b) -- (acc3c)node[midway, left]{$e_3$} -- (acc3d);
	%accolade
	\coordinate (acc4b) at (-0.5,-4.6); 
	\coordinate (acc4a) at (-0.3,-4.6); 
	\coordinate (acc4c) at (-0.5,-5.4); 
	\coordinate (acc4d) at (-0.3,-5.4); 
	\draw (acc4a) -- (acc4b) -- (acc4c)node[midway, left]{$e_4$} -- (acc4d);
	
\end{scope} 

\begin{scope}[shift = {(6,0)}]
	%NOEUDS
	\node[draw] (a) at (0,-1) {$\amessage_1$};
	\node[draw] (b) at (1.5,-1) {$\amessage_2$};
	
	%ARCS
	\draw[->] (a) -- (b)node[midway, above]{$SS$};
	
	%C	
	\node[text width=4cm,text centered] at(4.5,-1){
	  $\begin{array}{c@{\ =\ }c@{\quad}c@{\ =\ }c}
            C_{S,s} &   \emptyset & C'_{S,s} & \{q\} \\
            C_{R,s} & \emptyset & C'_{R,s} & \{t\}	
	\end{array}$};


	%NOEUDS
	\node[draw] (c) at (0,-2.5) {$\amessage_3$};
	\node[draw] (d) at (1.5,-2.5) {$\amessage_4$};	
	\node[draw] (e) at (-1.5,-2.3) {$\lambdanode_s$};
	
	%ARCS
	\draw[->] (c) -- (d)node[midway, above]{$RR$};
	\draw[->, dashed] (c) to[bend right = 50] node[midway, below]{$SS$} (d);
	\draw[->, dashed] (e) to[bend right = 20] node[midway, below]{$SS$} (c);
	
	%C
	\node[text width=4cm,text centered] at(4.3,-2.5){
	  $\begin{array}{c@{\ =\ }c@{\quad}c@{\ =\ }c}
            C_{S,s} & \{q\} & C'_{S,s} & \{q,t,u\} \\
            C_{R,s} & \{t\} & C'_{R,s} & \{t,p\}	
	\end{array}$};
	
	%NOEUDS
	\node[draw] (f) at (0,-4) {$\amessage_5$};
	\node[draw] (g) at (-1.5,-3.8) {$\lambdanode_s$};
	
	%ARCS
	\draw[->, dashed] (g) to[bend right = 20] node[midway, below]{$SR$} (f);
	
	%C
	\node[text width=4cm,text centered] at(4.3,-4){
	  $\begin{array}{c@{\ =\ }c@{\quad}c@{\ =\ }c}
            C_{S,s} & \{q,t,u\} & C'_{S,s} & \{q,t,u\} \\
            C_{R,s} & \{t,p\} & C'_{R,s} & \{t,p\}	
	\end{array}$};
	
	%NOEUDS
	\node[draw] (h) at (0,-5) {$\amessage_6$};
	\node[draw] (i) at (-1.5,-4.8) {$\lambdanode_s$};
	
	%ARCS
	\draw[->, dashed] (i) to[bend right = 20] node[midway, below]{$SS$} (h);
	
	%C
	\node[text width=4cm,text centered] at(4.3,-5){
	  $\begin{array}{c@{\ =\ }c@{\quad}c@{\ =\ }c}
            C_{S,s} & \{q,t,u\} & C'_{S,s} & \{q,t,u\} \\
            C_{R,s} & \{t,p\} & C'_{R,s} & \{t,p,s\}	
	\end{array}$};
	
	\end{scope} 

\end{tikzpicture} 

%\caption{MSC of execution $e$ and conflict graphs of its $\kE{k}s$}


==> proof-lem-feasible-bad.tex <==
% !TEX root = express19.tex 

Let us suppose $e'=e_1'\cdots e_n'$ be a \kSous{k} bad and feasible execution.
By Lemma \ref{lem:feasible-is-regular} we have that 
 there are
$B:\procSet\to2^{\procSet}$, 
$\finddest\in \procSet$, $C',\subseteq \procSet$, and a tuple of control states $\vec l'$ such that:
{\small
$$
(\vec l_0, B_0, \emptyset, \bot)
\transitionCD{e_1'}{k}\dots\transitionCD{e_n'}{k}
(\vec l', B', C', \destpi)
$$
}
We show that $$
(\vec l_0, B_0, \emptyset, \bot, \{\pi\},Q,\ctfalse,0)
\transitionBV{e_1'}{k}\dots\transitionBV{e_n'}{k}
(\vec l', B', C', \destpi, P',\{\pi\},\sawRS,\cont)
$$
for some $P'$,   $Q$
and 
either $\sawRS=\cttrue$, or $\cont=k+2$.

We proceed by induction on $n$.
\begin{description}
\item[Base n=2]
 Notice that,  for a feasible execution, there are at least two \kE{k} as the deviation cannot fit a sigle \kE{k}: the send from process $\pi$ to the original recipient must follow the reception of the deviated message, thus it has to belong to a subsequent \kE{k}.
 Then $e' = e_1' e_2'$.
 
 By Lemma \ref{lem:bad-characterization}, we have that either $\vstart\cgedge{}^*\cgedge{RS}\cgedge{}^*\vstop$, or 
%\item 
the size of the set $\succs{\vstart}\cap\preds{\vstop}$ is greater or equal to $k+2$.

If $\vstart\cgedge{}^*\cgedge{RS}\cgedge{}^*\vstop$, then since a label RS cannot exists in a local conflict graph
there exist two paths $\vstart\cgedge{}^*v_1$ in $\cgraph{e_1}$ and $v_2\cgedge{}^*\vstop$ in $\cgraph{e_2}$, with $\procofactionv{R}{v_1}$=$\procofactionv{S}{v_2}$.
We have that $v_2 \in \predse{e_2}{\pi} and $\lastisRec{\procofactionv{S}{v_2}}$ is $\cttrue$, thus $\sawRS$ becomes $\cttrue$ concluding this part of the proof.

Now suppose that  the size of the set $\succs{\vstart}\cap\preds{\vstop}$ is greater or equal to $k+2$. We show that all nodes in $\succs{\vstart}\cap\preds{\vstop}$ have been count either in the first or in the second \kE{k}.
 






\item[Inductive step]

\end{description}



 

==> relatedwork.tex <==
\section{Related Work}
$k$-synchronizability has been introduced in \cite{DBLP:conf/cav/BouajjaniEJQ18}, its principal interest is that a $k$-synchronizable system reaches the same global state with asynchronous communication as with synchronous communication. Moreover, in such a system, detecting deadlocks becomes decidable. Other properties close to it have been defined in the literature. Many of them, like $k$-synchronizability, concern system boundaries since reducing an asynchronous and unbounded system to a bounded communication can allow to make several problems decidable. 

%Existentially k-bounded
Some properties are related to the capacity of buffers. For example, in \cite{DBLP:conf/lata/Muscholl10} and \cite{genestcommunicating2007}, the authors study the fact that a system is existentially $k$-bounded. Overall, this means that for each execution of the system, there is a causally equivalent execution that has, at most and at any given time, $k$ messages not received in each buffer. A $k$-synchronizable system is existentially $k$-bounded \cite{lange2019verifying}. If a system is deadlock-free, decide if it is existentially $k$-bounded for a given $k$ is decidable.  

%K-exhaustivity 
Existentially bounded systems are compared in \cite{lange2019verifying} to $k$-exhaustive systems. A system is $k$-exhaustive if for all the configurations reachable in a $k$-bounded system, each time a sending action is allowed, then it can be executed in this system. 
The authors then note that a $k$-exhaustive system is existentially $k$-bounded. The $k$-exhaustivity is also compared to the $k$-synchronizability defined in \cite{DBLP:conf/cav/BouajjaniEJQ18}, a $k$-synchronizable system that has the property of eventual reception is $k$-exhaustive. This property ensures that any message sent can always be received. 
However, $k$-exhaustivity is only defined for peer-to-peer systems of communicating session automata, i.e., where each state of each automaton representing a process can only either send or receive.

%Universally et stability 
Another property, introduced in \cite{DBLP:conf/acsd/GenestM05}, is to check if each execution of the system can only be done with buffers of size $b$, the system is then universally $b$-bounded. Stability, defined in \cite{akroun2018automated}, is similar, it describes a system where the $b$-bounded behaviour is the same as the asynchronous behaviour. However, we can note that in \cite{DBLP:conf/acsd/GenestM05}, systems communicate within peer-to-peer communication and compare the entire trace  while the communication in \cite{akroun2018automated} is within mailbox and only send traces are looked at. 

%Synchronizability
If a system is stable, w.r.t \cite{akroun2018automated}, with a bound $b=1$ then the system is said to be synchronizable (same terminology as \cite{DBLP:conf/cav/BouajjaniEJQ18} but different in meaning). 
In \cite{finkel2017synchronizability}, the authors determine that synchronizability is, in general, not decidable for peer-to-peer systems. Some system topologies allow synchronizability to be decidable.

%Context switching
In \cite{DBLP:conf/tacas/TorreMP08}, the authors study the problem of reachability in communicating systems with a bounded number of context-switching. If $k$-synchronizability tends to limit the number of consecutive sending, limiting the number of context-switching is on the contrary to limit the number of times the actor process is changed, and therefore to optimize the number of consecutive actions performed by the same process.  
Only forest topology admits a decidable reachability problem for recursive programs. As for non-recursive programs, the problem is decidable for non-recursive systems with a polyforest topology.  
Like $k$-synchronizability, this problem applies to FIFO communicating systems on unbounded buffers, but they have peer-to-peer communication and not mailbox communication.




 


==> theorem.tex <==
\paragraph{\bf Decidability.}
%\cin{too quick here, we need a theorem and proof right?}
To know if a mailbox system $\system$ is \kSable{k}, we have to construct all possible \kE{k}s in system $\system'$ respecting the causal delivery and being \kSous{k} in $\system$. If a succession of \kE{k}s allows to reach a configuration with $\globalstate{l} = \error$ then the system is not \kSable{k}.  

%The set of such k-exchanges is finite. The reachability problem in a finite state machine is decidable. So the k-synchronizability for mailbox systems is decidable. 

\begin{lem}\label{lemma:finiteLTS}
The set of \kE{k}s into the \kSous{k} semantics of a system $\system'$ forms a finite-state labelled transition system (LTS).  
\end{lem}

\begin{proof}
Set $L_p$ for each $p \in \procSet$ is finite. Set $\procSet$ is finite and the result of function $B$ contains, for each process $p \in \procSet$, a finite set of processes so it is also finite. We can ignore the contains of $\B$ because each \kE{k} begins with $\B^{\emptyset}$. The result of function $C$ contains also a part of $\procSet$. The set $D$ contains tuples containing a process and a boolean, therefore there is also a finite number of possibilities for $D$. Finally, variable $count$ is an integer between $0$ and $k$, and $\findsend$ and $\findfrom$ are booleans. 

Therefore, the set of \kE{k}s is finite. The system formed by the set of \kE{k} and the possible transitions between us is so a finite-state LTS.  
\end{proof}

\begin{lem}\label{lemma:reachability}
The reachability problem into the \kSous{k} semantics of a system $\system'$ is decidable. 
\end{lem}

\begin{proof}
According to Lemma~\ref{lemma:finiteLTS}, the set of \kE{k}s in the \kSous{k} semantics of system $\system'$ forms a finite-state LTS. The reachability problem into a finite-state LTS is decidable. 
So the reachability problem into the \kSous{k} semantics of a system $\system'$ is decidable.      
\end{proof}

\begin{theorem}
The \kSity{k} is decidable for mailbox systems.
\end{theorem}

\begin{proof}
Decide if a system is not \kSable{k} means search a reachable \kE{k} with $\globalstate{l}= \error$. According to Lemma~\ref{lemma:reachability}, the reachability problem into the \kSous{k} semantics of system $\system'$ is decidable. So the \kSity{k} is decidable. 
\end{proof}




